AIBrix: Towards Scalable, Cost-Effective Large Language Model Inference Infrastructure

We introduce AIBrix, a cloud-native, open-source framework designed to optimize and simplify large-scale LLM deployment in cloud environments. Unlike traditional cloud-native stacks, AIBrix follows a co-design philosophy, ensuring every layer of the infrastructure is purpose-built for seamless integration with inference engines like vLLM. AIBrix introduces several key innovations to reduce inference costs and enhance performance including high-density LoRA management for dynamic adapter scheduling, LLM-specific autoscalers, and prefix-aware, load-aware routing. To further improve efficiency, AIBrix incorporates a distributed KV cache, boosting token reuse across nodes, leading to a 50% increase in throughput and a 70% reduction in inference latency. AIBrix also supports unified AI runtime which streamlines model management while maintaining vendor-agnostic engine compatibility. For large-scale multi-node inference, AIBrix employs hybrid orchestration -- leveraging Kubernetes for coarse-grained scheduling and Ray for fine-grained execution -- to balance efficiency and flexibility. Additionally, an SLO-driven GPU optimizer dynamically adjusts resource allocations, optimizing heterogeneous serving to maximize cost efficiency while maintaining service guarantees. Finally, AIBrix enhances system reliability with AI accelerator diagnostic tools, enabling automated failure detection and mock-up testing to improve fault resilience. AIBrix is available at https://github.com/vllm-project/aibrix.

==> text/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\subsection{Distributed KV Cache Pool}
Table~\ref{tab:eval_cache_performance_comparison}
\begin{table}[ht]
    \centering
    \scriptsize
    % \begin{tabular}{lcccccccccc}
    \begin{tabular}{>{\raggedright\arraybackslash}p{2cm} ccccccccc}
        \toprule
        & \multicolumn{2}{c}{Tokens} & \multicolumn{2}{c}{Throughput (tokens/sec)} & \multicolumn{2}{c}{TTFT (ms)} & \multicolumn{2}{c}{ITL (ms)} & \multicolumn{1}{c}{Completion} \\
        \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
        Method & Prompt & Decoding & Total & Decoding & Avg. & P99 & Avg. & P99 & Time (sec) \\
        \midrule
        vLLM Default & 1082837 & 12726 & 1,802.30 & 20.94 & 3,067.07 & 10,060.29 & 189.04 & 3,175.79 & 607.87 \\
        AIBrix Distributed KV Cache + Default & 1082837 & 12762 & 4,133.45 & 48.15 & 825.77 & 2,132.97 & 89.78 & 831.98 & 265.06 \\
        \textbf{Improvement} & & & 129.34\% & 129.98\% & 73.08\% & 78.80\% & 52.51\% & 73.80\% & 56.40\% \\
        \midrule
        vLLM Chunked Prefill & 1082837 & 12756 & 1,820.63 & 21.20 & 4,500.58 & 12,411.33 & 164.41 & 288.77 & 601.77 \\
        AIBrix Distributed KV Cache + Chunked Prefill & 1082837 & 12744 & 3,320.91 & 38.63 & 2,235.12 & 6,151.27 & 93.34 & 151.68 & 329.90 \\
        \textbf{Improvement} & & & 82.40\% & 82.23\% & 50.34\% & 50.44\% & 43.23\% & 47.47\% & 45.18\% \\
        \midrule
        vLLM Prefix Caching & 1082837 & 12775 & 3,703.26 & 43.18 & 999.95 & 5,744.27 & 99.50 & 1,653.56 & 295.85 \\
        AIBrix Distributed KV Cache + Prefix Caching & 1082837 & 12761 & 5,615.71 & 65.41 & 349.39 & 1,306.05 & 69.95 & 456.31 & 195.10 \\
        \textbf{Improvement} & & & 51.64\% & 51.48\% & 65.06\% & 77.26\% & 29.70\% & 72.40\% & 34.06\% \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison of vLLM and \sysname{} Distributed KV Cache with different configurations. Here the vLLM Default is the configuration with chunked prefill and prefix caching disabled}
    \label{tab:eval_cache_performance_comparison}
\end{table}

\subsection{Cost-Efficient and SLO-Driven Heterogeneous Serving}


\subsection{Autoscaling}
Figure~\ref{fig:eval-autoscaling}
\begin{figure}[ht]%
    \centering
    \subfloat[\centering \textit{Average number of replicas.}]{{\includegraphics[width=.2\columnwidth]{plot/autoscaling/replicas-line.png}}\label{fig:eval-autoscaling-replicas}}
    \hfill
    \subfloat[\centering \textit{Average latency.}]{{\includegraphics[width=.2\columnwidth]{plot/autoscaling/latency-line.png}}\label{fig:eval-autoscaling-latency}}
    \hfill
    \subfloat[\centering \textit{Average RPS. }]{{\includegraphics[width=.2\columnwidth]{plot/autoscaling/rps-line.png}}\label{fig:eval-autoscaling-rps}}
    \hfill
    \subfloat[\centering \textit{Average Throughput.}]{{\includegraphics[width=.2\columnwidth]{plot/autoscaling/throughput-line.png}}\label{fig:eval-autoscaling-throughput}}
    \subfloat[\centering \textit{Average prompt tokens.}]{{\includegraphics[width=.2\columnwidth]{plot/autoscaling/prompt-tokens-line.png}}\label{fig:eval-autoscaling-prompt-tokens}}
    \caption{\textit{HPA vs. KPA}}
    \label{fig:eval-autoscaling}
\end{figure}



\subsection{GPU Streaming Loader}




% \begin{table}[h]
%     \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Feature} & \textbf{AIBrix Model Loader} & \textbf{Tensorizer} & \textbf{vLLM Default (Transformer/HuggingFace Hub)} \\
%         \midrule
%         File Format: Safetensor Support & \checkmark & $\times$ (Requires Custom Storage Format) &  \checkmark \\
%         \midrule
%         \multicolumn{4}{l}{\textbf{Storage Support}} \\
%         Local Disk &  \checkmark &  \checkmark &  \checkmark \\
%         S3 &  \checkmark &  \checkmark & $\times$ \\
%         TOS &  \checkmark & $\times$ & $\times$ \\
%         HuggingFace & $\times$ & $\times$ & \checkmark \\
%         \midrule
%         Loading Acceleration & 10\%+ & Different mechanisms, not comparable & Baseline \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison of Model Loaders}
%     \label{tab:model_loader_comparison}
% \end{table}

% \begin{table}[h]
%     \centering
%     \setlength{\tabcolsep}{5pt} % Adjust column spacing
%     \renewcommand{\arraystretch}{1.2} % Adjust row height
%     \begin{tabular}{>{\raggedright\arraybackslash}p{4cm} >{\centering\arraybackslash}p{3cm} >{\centering\arraybackslash}p{3cm} >{\centering\arraybackslash}p{4cm}}
%         \toprule
%         \textbf{Feature} & \textbf{AIBrix Model Loader} & \textbf{Tensorizer} & \textbf{vLLM Default (Transformer/HuggingFace Hub)} \\
%         \midrule
%         File Format: Safetensor Support & \checkmark & $\times$ (Requires Custom Storage Format) & \checkmark \\
%         \midrule
%         \multicolumn{4}{l}{\textbf{Storage Support}} \\
%         Local Disk & \checkmark & \checkmark & \checkmark \\
%         S3 & \checkmark & \checkmark & $\times$ \\
%         TOS & \checkmark & $\times$ & $\times$ \\
%         HuggingFace & $\times$ & $\times$ & \checkmark \\
%         \midrule
%         Loading Acceleration & 10\%+ & Different mechanisms, not comparable & Baseline \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison of Model Loaders}
%     \label{tab:eval_model_loader_comparison}
% \end{table}


\subsection{Advanced LLM Gateway and Routing Strategies}

